Ergodicity and Mixing of Sublinear Expectation System and Applications

We utilize an ergodic theory framework to explore sublinear expectation theory. Specifically, we investigate the pointwise Birkhoff's ergodic theorem for invariant sublinear expectation systems. By further assuming that these sublinear expectation systems are ergodic, we derive stronger results. Furthermore, we relax the conditions for the law of large numbers and the strong law of large numbers under sublinear expectations from independent and identical distribution to $\alpha$-mixing. These results can be applied to a class of stochastic differential equations driven by $G$-Brownian motion (i.e., $G$-SDEs), such as $G$-Ornstein-Uhlenbeck processes. As byproducts, we also obtain a series of applications for classical ergodic theory and capacity theory.

==> symbols.tex <==
\def \a{\alpha} 
\def \b{\beta} 
\def \g{\gamma} 
\def \d{\delta}
\def \t{\theta} 
\def \T{\Theta} 
\def \p{\Theta} 
\def \e{\epsilon}
\def \s{\sigma} 
\def \l{\lambda} 
\def \z{\zeta} 
\def \o{\omega}
\def \O{\Omega} 
\def \D{\Delta} 
\def \F{\mathscr{F}} 
\def \r{\rho}
\def \k{\kappa} 
\def \Si{\Sigma} 
\def \G{\Gamma}
\def \di{\mathrm{dist}} 
\def \spa{\mathrm{span}}
\def \pa{\partial} \def\an{\measuredangle}
\def \L{\Lambda}
\def\deq{\stackrel{d}{=}}
\def\one{\mathbf 1}


